Fingerprint Presentation Attack Detection: A Sensor and Material Agnostic Approach

The vulnerability of automated fingerprint recognition systems to presentation attacks (PA), i.e., spoof or altered fingers, has been a growing concern, warranting the development of accurate and efficient presentation attack detection (PAD) methods. However, one major limitation of the existing PAD solutions is their poor generalization to new PA materials and fingerprint sensors, not used in training. In this study, we propose a robust PAD solution with improved cross-material and cross-sensor generalization. Specifically, we build on top of any CNN-based architecture trained for fingerprint spoof detection combined with cross-material spoof generalization using a style transfer network wrapper. We also incorporate adversarial representation learning (ARL) in deep neural networks (DNN) to learn sensor and material invariant representations for PAD. Experimental results on LivDet 2015 and 2017 public domain datasets exhibit the effectiveness of the proposed approach.

==> Fingerprint Spoof Detection_ Cross-Sensor Generalization/algo.tex <==
Algorithm 1 Training UMG wrapper
1: procedure
2: input
3: x: source image providing friction ridge content and
known style A
4: y: target image providing known style B
5: f(·): encoder network; first 4 layers of VGG-19 network pre-trained on ImageNet with weights frozen during
training
6: g(·): decoder network; mirrors f(·) with pooling layers
replaced with nearest up-sampling layers
7: D(·): discriminator function similar to [38]
8: A(x, y): AdaIN operation; transfer style from x to y
(using Eq. 2)
9: α = 0.5
10: λc = 0.001, λs = 0.002
11: output
12: UMG(·): UMG wrapper trained on known materials
13: begin:
14: Encoding: fx = f(x) and fy = f(y)
15: Style transfer: t = A(fx, fy)
16: Stylized image: T(c, s, α) = g((1 − α) · fc + α · t)
17: Style Loss: Ls using Eq. 4
18: Content Loss: Lc using Eq. 6
19: Adversarial Loss (generator): L
G
adv using Eq. 7
20: Adversarial Loss (discriminator): L
D
adv using Eq. 8
21: Objective functions for training UMG wrapper
22: minG LG = λc · Lc + λs · Ls + L
G
adv
23: maxD LD = L
D
adv
24: end


D^{real}_{Source} = {D^{real}_SA, D^{real}_SB, D^{real}_SC}

D^{real}_{Target} = D^{real}_SD

D^{synth}_{Target}

D^{synth}_{Target} = UMG(D^{real}_{Source}, D^{real}_{Target})

D_Train = {D^{real}_{Source}, D^{real}_{Target}, D^{synth}_{Target}}

Training A CNN on D_Train
- Three losses
- minimax game



1. Tarang

Combine figures to make proposed approach with all individual parts % done

Change Figure 3 to make it compact with different patches % not required now

Add algorithm with data and losses defined // assuming UMG is referenced
% in progress

2. Steve

Section 3.2 explain three losses with  obvious equations
 talk about encoder, decoder,, etc. %done
 
 section 3.6 
 explicitly mention the advantages of fusing two approaches %done
 add algorithm %I believe you will add this


4.3 implementation details

mention the encoder and target predictor and adversary architecture %done



==> algo.tex <==
Algorithm 1 Training UMG wrapper
1: procedure
2: input
3: x: source image providing friction ridge content and
known style A
4: y: target image providing known style B
5: f(·): encoder network; first 4 layers of VGG-19 network pre-trained on ImageNet with weights frozen during
training
6: g(·): decoder network; mirrors f(·) with pooling layers
replaced with nearest up-sampling layers
7: D(·): discriminator function similar to [38]
8: A(x, y): AdaIN operation; transfer style from x to y
(using Eq. 2)
9: α = 0.5
10: λc = 0.001, λs = 0.002
11: output
12: UMG(·): UMG wrapper trained on known materials
13: begin:
14: Encoding: fx = f(x) and fy = f(y)
15: Style transfer: t = A(fx, fy)
16: Stylized image: T(c, s, α) = g((1 − α) · fc + α · t)
17: Style Loss: Ls using Eq. 4
18: Content Loss: Lc using Eq. 6
19: Adversarial Loss (generator): L
G
adv using Eq. 7
20: Adversarial Loss (discriminator): L
D
adv using Eq. 8
21: Objective functions for training UMG wrapper
22: minG LG = λc · Lc + λs · Ls + L
G
adv
23: maxD LD = L
D
adv
24: end


D^{real}_{Source} = {D^{real}_SA, D^{real}_SB, D^{real}_SC}

D^{real}_{Target} = D^{real}_SD

D^{synth}_{Target}

D^{synth}_{Target} = UMG(D^{real}_{Source}, D^{real}_{Target})

D_Train = {D^{real}_{Source}, D^{real}_{Target}, D^{synth}_{Target}}

Training A CNN on D_Train
- Three losses
- minimax game



1. Tarang

Combine figures to make proposed approach with all individual parts % done

Change Figure 3 to make it compact with different patches % not required now

Add algorithm with data and losses defined // assuming UMG is referenced
% in progress

2. Steve

Section 3.2 explain three losses with  obvious equations
 talk about encoder, decoder,, etc. %done
 
 section 3.6 
 explicitly mention the advantages of fusing two approaches %done
 add algorithm %I believe you will add this


4.3 implementation details

mention the encoder and target predictor and adversary architecture %done


